Fair treatment allocations in social networks

Simulations of infectious disease spread have long been used to understand how epidemics evolve and how to effectively treat them. However, comparatively little attention has been paid to understanding the fairness implications of different treatment strategies -- that is, how might such strategies distribute the expected disease burden differentially across various subgroups or communities in the population? In this work, we define the precision disease control problem -- the problem of optimally allocating vaccines in a social network in a step-by-step fashion -- and we use the ML Fairness Gym to simulate epidemic control and study it from both an efficiency and fairness perspective. We then present an exploratory analysis of several different environments and discuss the fairness implications of different treatment strategies.

==> formal_problem.tex <==
\section{Problem Statement}
Let $K = \{1, ..., N_p\}$ be indices that represent individual members of a population with $N_p$ members and let $N_t$ be the number of treatments an agent can give out.  Let $A \in P^{N_t}$ be an allocation of treatments to individuals in the population.  Finally, let $H = \{S,I,R\}^{N_p}$ be a health state, and let $\tau$ be a schedule according to which treatments are given out -- perhaps only at $t=0$, or at timestep, or something else.

The agent's task is to find a probabilistic \emph{allocation policy} $f: H \rightarrow P(A)$ that maps health states to a distribution over allocations.  This function will be applied according to the schedule $\tau$.  One way to go about this is to find the policy by solving an optimization problem that encodes a goal related to reducing infection.

A few more definitions are required before we pose the optimization problems.  Let $x_i | t, f \in \{0, 1\}$ be a random variable that indicates whether individual $i \in K$ ever enters the \texttt{Infected} state by time $t$ given allocation policy $f$.

Now consider an agent whose only concern is to maximize utility -- that is, to minimize the number of individuals who get sick once the infectious disease has played out.  They can find this \emph{maximum utility} policy by solving the following optimization problem:
\begin{equation}
\begin{aligned}
f_{MU} = \argmin_{f} \quad & \frac{1}{N_p} \sum\limits_{i=1}^{N_p} P(x_i = 1 | t=\infty, f) \\
\end{aligned}
\end{equation}

Consider now an agent who is concerned with a particular notion of fairness -- each member of the population should have the same probability of being infected.  An agent can find this \emph{naively equitable} policy by adding a constraint to the problem above:
\begin{equation}
\begin{aligned}
f_{NE} = \argmin_{f} \quad & \frac{1}{N_p} \sum\limits_{i=1}^{N_p} P(x_i = 1 | t=\infty, f) \\
\textrm{s.t.} \quad & P(x_i = 1 | t=\infty, f) = P(x_j = 1 | t=\infty, f) \: \forall \: i, j \in K
\end{aligned}
\end{equation}

Why is the policy naive?  It could well be the case that there's a policy that \emph{dominates} the naively equitable policy by offering an improvement for every individual over the naively equitable policy.  That is, an \emph{undominated equitable} policy is a naively equitable policy for which:
\begin{equation}
\nexists f' \; \textrm{s.t.} \; P(x_i = 1 | t=\infty, f') < P(x_j = 1 | t=\infty, f) \: \forall \: i \in K
\end{equation}

==> related_work.tex <==
\section{Related Work}
In this section, we provide a brief overview of infectious disease modeling.

\subsection{Infectious Disease Epidemiology}

Infectious disease epidemiology studies infectious disease at the population level.  Researchers in this field rely on simple models where human contact is associated with some probability of communicating disease.  Compartmental models, which are a central to the study, represent disease dynamics in populations by specifying a small number of mutually exclusive states that members of a population can occupy and some kind of mechanism by which disease propagates \cite{hethcote2000mathematics}.

In this paper, we study the Susceptible-Exposed-Infected-Recovered (SEIR) subclass of compartmental models, where individuals exist in one of four mutually exclusive states: \texttt{Susceptible}, \texttt{Exposed}, \texttt{Infected}, and \texttt{Recovered}.  \texttt{Susceptible} people are healthy but vulnerable to infection, \texttt{Exposed} people are not yet sick but will become so after time passes, \texttt{Infected} people are sick and spreading the disease, and \texttt{Recovered} people were once sick but no longer are.  Note that not all stages need be present -- for example, the SI model only includes the \texttt{Susceptible} and \texttt{Infected} states.

Compartmental models are not fully specified by the states that people can occupy.  Additional considerations include the representation of time, which is typically treated as continuous, but the discrete case is actively studied as well (such as in \cite{brauer2010discrete,hernandez2015discrete,liu2015effect,allen1994some}).  

In addition, there is the question of how people come into contact.  Models typically assume `full mixing,' whereby all members of a population are equally likely to come into contact with all other members of a population.  However, there is a rich vein of work that assumes instead that contact proceeds along some explicitly-specified social network (for a detailed treatment, see \cite{newman2002spread, newman2018networks}).

